Machine-Learning-Driven Runtime Optimization of BLAS Level 3 on Modern Multi-Core Systems

BLAS Level 3 operations are essential for scientific computing, but finding the optimal number of threads for multi-threaded implementations on modern multi-core systems is challenging. We present an extension to the Architecture and Data-Structure Aware Linear Algebra (ADSALA) library that uses machine learning to optimize the runtime of all BLAS Level 3 operations. Our method predicts the best number of threads for each operation based on the matrix dimensions and the system architecture. We test our method on two HPC platforms with Intel and AMD processors, using MKL and BLIS as baseline BLAS implementations. We achieve speedups of 1.5 to 3.0 for all operations, compared to using the maximum number of threads. We also analyze the runtime patterns of different BLAS operations and explain the sources of speedup. Our work shows the effectiveness and generality of the ADSALA approach for optimizing BLAS routines on modern multi-core systems.

==> Ideal_performance.tex <==
\begin{tabular}{l|l|ll}
    % \toprule
    & {} & 0-100M & 0-500M \\
    \midrule
    \multirow{ 2}{0.20\columnwidth}{\textbf{${\text{Speedup-ideal}}$}}& Gadi (Intel) &      1.61 &        1.12 \\
    \cmidrule{2-2}
    & ParaTera (AMD) &      1.82 &        - \\
    \midrule
    \multirow{ 2}{0.15\columnwidth}{\textbf{${\text{Speedup-model}}$}}& Gadi  &      1.45 &        1.04 \\
    \cmidrule{2-2}
    & ParaTera &    1.51   &        - \\
    \midrule
    \multirow{ 2}{0.15\columnwidth}{\textbf{${\text{Speedup}}$}}& Gadi  &      1.32 &        1.01 \\
    \cmidrule{2-2}
    & ParaTera &      - &        - \\
    \bottomrule
\end{tabular}

==> estimated_speedup.tex <==
\begin{tabularx}{\textwidth}{lXXXXXXXXX}
    \toprule
    {} &  Model &    test\_rmse(1e-6s) &  ideal\_speedup\_mean &  ideal\_speedup\_sum  &  eval\_time(1e-6s) &  estimated\_speedup\_mean &  estimated\_speedup\_sum \\
    \midrule
    1 &  Linear Regression &       97984.89 &                1.19 &                   1.03  &           42.94 &                    1.18 &                       1.03 \\
    2 &  ElasticNet &     100702.16 &                1.08 &                   0.90  &           24.98 &                    1.08 &                       0.90 \\
    3 &  Bayes Regression &       97984.90 &                1.19 &                   1.03  &            7.91 &                    1.19 &                       1.03 \\
    4 &  Decision Tree &       28031.94 &                0.50 &                   0.50  &            11.07 &                   0.50 &                   0.50 \\
    5 &  Random Forest &       18602.57 &                1.58 &                   1.43  &        20816.25 &                    0.76 &                       0.83 \\
    6 &  AdaBoost &       42585.91 &                0.55 &                   0.57  &          133.11 &                    0.55 &                       0.56 \\
    7 &  XGBoost &       {12750.74} &                {1.50} &                   1.38  &          45.02 &                    1.50 &                       1.37 \\
    8 &  kNN &   25709.83 &                1.70 &                   1.52  &        35173.48 &                    0.61 &                       0.66 \\
    \bottomrule
\end{tabularx}

==> machines.tex <==

{
%\scriptsize
\sffamily

\begin{tabular}{r@{\hspace{1.5ex}}r@{\hspace{1.5ex}}r@{\hspace{1.5ex}}r}%@{}r@{\hspace{1.5ex}}r@{\hspace{1.5ex}}r@{\hspace{1.5ex}}r@{} }
%\toprule
\\[-2ex]
{\textbf{Architecture}} & \multicolumn{1}{r@{\hspace{1.5ex}}}{\textbf{Pentium 4}} &  \multicolumn{1}{r@{\hspace{1.5ex}}}{\textbf{Atom D510}} & \multicolumn{1}{r}{\textbf{\sandy}} \\
\midrule 
{\textbf{Model}} & 
P4D 820 & Atom D510 & Core i7-2600 \\
{\textbf{Technology}} & 
90nm & 45nm & 32nm \\
{\textbf{Clock}} & 
2.8GHz & 1.66GHz & 3.4GHz \\
{\textbf{Cores $\times$ SMT}} &
2 $\times$ 2 & 2 $\times$ 2 & 4 $\times$ 2 \\
{\textbf{L2 Cache}} &
1MB $\times$ 2 & 512KB $\times$ 2 & 256KB $\times$ 4 \\ 
{\textbf{L3 Cache}} & 
none & none &  8MB\\
{\textbf{Memory}} & 
1GB DDR2-400 &  2GB DDR2-800  &  4GB DDR3-1066 \\

\bottomrule
\end{tabular}
}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> model_comp_time.tex <==

{
    %\scriptsize
    % \sffamily
    
    \begin{tabular}{p{0.15\columnwidth}|p{0.15\columnwidth}|p{0.15\columnwidth}|p{0.15\columnwidth}|p{0.15\columnwidth}}
    
    %\toprule
    {\textbf{Model Catagories}} & {\textbf{Models}} &  {\textbf{Training Time (ms)}} & {\textbf{Evaluation Time (ms)}} & {\textbf{Test RMSE}} \\
    \midrule
    \multirow{ 6}{0.15\columnwidth}{\textbf{Linear Models}} & Linear Regression & \multirow{ 2}{0.15\columnwidth}{12.8} & \multirow{ 2}{0.15\columnwidth}{2.1} & \multirow{ 2}{0.15\columnwidth}{5855.2} \\
    \cmidrule{2-5}
    & ElasticNet & {217.4} & 1.9 & 5983.9  \\
    \cmidrule{2-5}
    & Bayesian Regression & \multirow{ 2}{0.15\columnwidth}{26.2} & \multirow{ 2}{0.15\columnwidth}{1.9} & \multirow{2}{0.15\columnwidth}{5855.2} \\
    \midrule
    \multirow{ 7}{0.15\columnwidth}{\textbf{Tree Based Models}} & Decision Tree &  \multirow{2}{0.15\columnwidth}{214.6} & \multirow{2}{0.15\columnwidth}{2.0} & \multirow{2}{0.15\columnwidth}{7902.0} \\
    \cmidrule{2-5}
    & AdaBoost & 4250.9 & 32.4 & 4957.8 \\
    \cmidrule{2-5}
    & Random Forest & \multirow{2}{0.15\columnwidth}{4489.1} & \multirow{2}{0.15\columnwidth}{64.4} & \multirow{2}{0.15\columnwidth}{2256.3} \\
    \cmidrule{2-5}
    & XGBoost & 2623.6 & 18.4 & \text{1893.6} \\
    \cmidrule{2-5}
    & LightGBM & 1144.9 & 106.7 &  2857.1 \\
    \midrule
    \multirow{ 4}{0.15\columnwidth}{\textbf{Other Models}} & SVM Regressor & \multirow{2}{0.15\columnwidth}{3826.6} & \multirow{2}{0.15\columnwidth}{991.4} & \multirow{2}{0.15\columnwidth}{11747.2}\\
    \cmidrule{2-5}
    & KNN Regressor & \multirow{2}{0.15\columnwidth}{71.3} & \multirow{2}{0.15\columnwidth}{2533.4} & \multirow{2}{0.15\columnwidth}{2703.7}\\
    
    \bottomrule
    \end{tabular}
    }
    %%% Local Variables: 
    %%% mode: latex
    %%% TeX-master: t
    %%% End: 
    

==> performance_stats.tex <==
\scriptsize
\sffamily


\begin{tabular}{LSSSS}
    \toprule
     {} & \textbf{Setonix 0-500 MB} & \textbf{Setonix 0-100 MB} & \textbf{Gadi 0-500 MB} & \textbf{Gadi 0-100 MB}\\
    \midrule
    {\textbf{${\text{Mean Speedup}}$}}              &    1.32  &     {1.41}     &   1.07    &   1.26             \\
    {\textbf{${\text{Standard Deviation}}$}}& {0.41}    &   0.21     &     0.70     &    0.28                \\
    \midrule
    {\textbf{${\text{Min Speedup}}$}}               &  0.76    &   {0.87}       &   0.88    &    0.97                \\
    {\textbf{${\text{25th Percentile}}$}}   &   1.05  &   {1.17}        &   1.00    &      1.01           \\
    {\textbf{${\text{50th Percentile}}$}}   &  1.18   &    {1.29}       &   1.00    &      1.17              \\
    {\textbf{${\text{75th Percentile}}$}}   &  1.37     &   {1.61}      &   1.02    &       1.40             \\
    {\textbf{${\text{Max Speedup}}$}}      &    9.05      &    {2.49}        &   3.01    &       1.98                 \\
    \bottomrule
\end{tabular}

==> performance_stats_no_HT.tex <==
\scriptsize
\sffamily


\begin{tabular}{LSSSS}
    \toprule
     {} & \textbf{Setonix 0-500 MB} & \textbf{Setonix 0-100 MB} & \textbf{Gadi 0-500 MB} & \textbf{Gadi 0-100 MB}\\
    \midrule
    {\textbf{${\text{Mean Speedup}}$}}              &    1.24  &     {1.55}     &   1.02    &   1.34             \\
    {\textbf{${\text{Standard Deviation}}$}}& {0.58}    &   0.72     &     0.24     &    0.83                \\
    \midrule
    {\textbf{${\text{Min Speedup}}$}}               &  0.23    &   {0.60}       &   0.52    &    0.55                \\
    {\textbf{${\text{25th Percentile}}$}}   &   0.91  &   {1.16}        &   0.96    &      0.95           \\
    {\textbf{${\text{50th Percentile}}$}}   &  1.09   &    {1.39}       &   0.99    &      1.08              \\
    {\textbf{${\text{75th Percentile}}$}}   &  1.41     &   {1.75}      &   1.01    &       1.42             \\
    {\textbf{${\text{Max Speedup}}$}}      &    6.15      &    {8.54}        &   3.88    &       7.53                 \\
    \bottomrule
\end{tabular}

==> predictor_algo.tex <==
\begin{algorithm}
    \caption{ML Predictor Design}\label{Predictor Algo}
    \begin{algorithmic}[1]
    \Variables
    \State $\text{Booster Model}$
    \State $\text{Input Matrix}$
    \State $\text{Number Of Cores}$
    \State $\text{Chosen Features}$
    \State $\text{Data Transformer}$
    \State $\text{Data Normalizer}$
    \EndVariables
    \Procedure{Get optimal number of cores}{m, k, n}
    \For{$i$ \textbf{in} \textit{range}(0, Number Of Cores)}
    \State $\text{Input Matrix}$.$\textit{addRow}$(m, k, n, i)//construct a input matrix
    \EndFor
    \For {feature \textbf{in} $\text{Chosen Features}$}
    \State $\text{Input Matrix}$.$\textit{addFeature}$(feature)//construct needed features
    \EndFor
    \State $\text{Data Transformer}$.$\textit{transform}$($\text{Input Matrix}$)//Data transformation
    \State $\text{Data Normalizer}$.$\textit{normalize}$($\text{Input Matrix}$)//data normalization
    \State resultArray = $\text{Booster Model}$.\textit{predict}($\text{Input Matrix}$)//do the prediction
    \State \Return \textit{argmin}(resultArray) //return the number of threads with the least time
    \EndProcedure
    \end{algorithmic}
\end{algorithm}
  

==> raw_features.tex <==

{
%\scriptsize
\sffamily

\begin{tabular}{r@{\hspace{3ex}}r@{\hspace{3ex}}r@{\hspace{3ex}}r@{\hspace{3ex}}r}%@{}r@{\hspace{1.5ex}}r@{\hspace{1.5ex}}r@{\hspace{1.5ex}}r@{} }
\toprule
\\[-2ex]
$m$ & $k$ & $n$ & $"num\ of\ threads"$ \\

\bottomrule
\end{tabular}
}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

